Towards MoE Deployment: Mitigating Inefficiencies in Mixture-of-Expert (MoE) Inference

Mixture-of-Experts (MoE) models have gained popularity in achieving state-of-the-art performance in a wide range of tasks in computer vision and natural language processing. They effectively expand the model capacity while incurring a minimal increase in computation cost during training. However, deploying such models for inference is difficult due to their large size and complex communication pattern. In this work, we provide a characterization of two MoE workloads, namely Language Modeling (LM) and Machine Translation (MT) and identify their sources of inefficiencies at deployment. We propose three optimization techniques to mitigate sources of inefficiencies, namely (1) Dynamic gating, (2) Expert Buffering, and (3) Expert load balancing. We show that dynamic gating improves maximum throughput by 6.21-11.23$\times$ for LM, 5.75-10.98$\times$ for MT Encoder and 2.58-5.71$\times$ for MT Decoder. It also reduces memory usage by up to 1.36$\times$ for LM and up to 1.1$\times$ for MT. We further propose Expert Buffering, a new caching mechanism that only keeps hot, active experts in GPU memory while buffering the rest in CPU memory. This reduces static memory allocation by up to 1.47$\times$. We finally propose a load balancing methodology that provides additional scalability to the workload.

==> figures/scripts/dynamicspeedlm.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.48\textwidth]{figures/figures/dynamicspeedlm2.png}
\caption{{Latency comparison of different gating policies in MoE models, including static gating (baseline), Tutel gating\cite{tutel}, our dynamic gating policy, dynamic gating with Load Balancing (LB), dynamic gating with Expert Buffering (EB), and all optimizations combined. Missing bars represent infeasible cases under the corresponding policy and batch size. Eg. Tutel cannot support beyond batch size=32 for LM.
Dynamic gating reduces memory usage, enabling larger batch sizes and substantially faster processing times than static gating. Expert buffering trades latency for smaller memory usage while still achieving higher throughput on the MT Decoder. Load balancing further improves latency when combined with dynamic gating and expert buffering. Note that load balancing only makes sense in the context of dynamic gating where each expert gets different number of tokens. However the latency saving is marginal as difference in time between best and worst load is very small. Load balancing particularly shines when combined with expert buffering as it will be operating in a memory-intensive regime and it can improve cache miss rate (See Fig~\ref{fig:loadfix}).}}
\label{fig:dynamicspeedlm}
\end{figure}

%Dynamic gating also reduces the memory usage, therefore allowing a larger batchsize. Furthermore, Dynamic Gating is substantially faster than static gating, and load balancing speed it up further. While expert buffering trades the latency for a smaller memory usage, it is still capable to achieve a higher throughput on the MT Decoder.

==> figures/scripts/memory-breakdown.tex <==
\begin{figure*}[tbp]
\centering
\begin{subfigure}
  \centering
  \includegraphics[width=0.49\linewidth]{figures/figures/Language Model (1 Node, 8 GPUs).png}
  %\caption{}
  %\label{fig:moe-vs-dense-all}
\end{subfigure}%
\begin{subfigure}
  \centering
  \includegraphics[width=0.47\linewidth]{figures/figures/Machine Translation Model (1 Node, 8 GPUs).png}
  %\caption{}
  %\label{fig:moe-vs-dense-breakdown}
\end{subfigure}
\caption{Static memory usage breakdown for (left) language model and (right) machine translation model (using 1 node and 8 V100 GPU devices).}
\label{fig:memory-breakdown}
\end{figure*}

==> figures/scripts/motivation.tex <==
\begin{figure}[tbp]
\centering
\includegraphics[width=.48\textwidth]{figures/figures/scaling_trend.png}
\caption{\textcolor{red}{FIXME: This is not the motivation paper we want, we need a motivation figure that demonstrates whether M} Deep learning in general and deep learning based language model in particular have witnessed an exponential growth in parameter size in recent years~\cite{sevilla2022compute, newmoore2021}.
Note the difference in the growth trend across different domains.}
\label{fig:motivation}
\end{figure}

